Learning Enhanced Structural Representations with Block-Based Uncertainties for Ocean Floor Mapping

Accurate ocean modeling and coastal hazard prediction depend on high-resolution bathymetric data; yet, current worldwide datasets are too coarse for exact numerical simulations. While recent deep learning advances have improved earth observation data resolution, existing methods struggle with the unique challenges of producing detailed ocean floor maps, especially in maintaining physical structure consistency and quantifying uncertainties. This work presents a novel uncertainty-aware mechanism using spatial blocks to efficiently capture local bathymetric complexity based on block-based conformal prediction. Using the Vector Quantized Variational Autoencoder (VQ-VAE) architecture, the integration of this uncertainty quantification framework yields spatially adaptive confidence estimates while preserving topographical features via discrete latent representations. With smaller uncertainty widths in well-characterized areas and appropriately larger bounds in areas of complex seafloor structures, the block-based design adapts uncertainty estimates to local bathymetric complexity. Compared to conventional techniques, experimental results over several ocean regions show notable increases in both reconstruction quality and uncertainty estimation reliability. This framework increases the reliability of bathymetric reconstructions by preserving structural integrity while offering spatially adaptive uncertainty estimates, so opening the path for more solid climate modeling and coastal hazard assessment.

==> lemmas.tex <==
\section{Appendix}

\subsection{Block-wise vs Global Uncertainty Analysis}

\begin{lemma}[Block-wise Error Distribution]
\label{lemma-block-error}
Let $\mathcal{B} = \{b_1, ..., b_N\}$ be a partition of the bathymetric space into blocks, and let:
\begin{itemize}
    \item $\sigma^2_i$ be the error variance in block $i$
    \item $\sigma^2_g$ be the global error variance
    \item $c_i$ be the complexity measure of block $i$
    \item $\kappa_i = c_i/\sum_j c_j$ be the normalized complexity
\end{itemize}
Then the following inequality holds:
\begin{equation}
    \sum_{i=1}^N \kappa_i\sigma^2_i \leq \sigma^2_g
\end{equation}
with equality if and only if all blocks have identical complexity and error characteristics.
\end{lemma}

\begin{proof}
The global variance can be decomposed as:
\begin{equation}
    \sigma^2_g = \frac{1}{|\mathcal{X}|}\sum_{x \in \mathcal{X}}(f(x) - \hat{f}(x))^2
\end{equation}
where $\mathcal{X}$ is the full domain.

For block-wise variances:
\begin{equation}
    \sigma^2_i = \frac{1}{|b_i|}\sum_{x \in b_i}(f(x) - \hat{f}(x))^2
\end{equation}

The inequality follows from Jensen's inequality and the fact that error variance typically increases with complexity. 
\end{proof}

\begin{theorem}[Block-wise vs Global Loss Optimization]
\label{theorem-block-loss}
Let $\mathcal{L}_B$ be the block-wise uncertainty-weighted loss and $\mathcal{L}_G$ be the global uncertainty-weighted loss:
\begin{align}
    \mathcal{L}_B &= \sum_{i=1}^N U_i \cdot |D(z_q)_i - x_i|^2 \\
    \mathcal{L}_G &= U_g \cdot \sum_{i=1}^N |D(z_q)_i - x_i|^2
\end{align}
where $U_i$ is the block-wise uncertainty and $U_g$ is the global uncertainty.

For any local feature scale $F$ and correlation length $C$, the block-wise loss leads to better reconstruction of local features:
\begin{equation}
    \mathbb{E}[\|\nabla f - \nabla \hat{f}_B\|_2^2] \leq \mathbb{E}[\|\nabla f - \nabla \hat{f}_G\|_2^2]
\end{equation}
where $\hat{f}_B$ and $\hat{f}_G$ are reconstructions optimized with block-wise and global losses respectively.
\end{theorem}

\begin{proof}
Let $\mathcal{H}_i$ be the set of high-frequency features in block $i$. The block-wise loss allows for adaptive weighting:
\begin{equation}
    U_i \propto |\mathcal{H}_i| / |b_i|
\end{equation}

For the global case, the uncertainty is averaged:
\begin{equation}
    U_g = \frac{1}{N}\sum_{i=1}^N \frac{|\mathcal{H}_i|}{|b_i|}
\end{equation}

This leads to suboptimal weighting for blocks with:
\begin{equation}
    |\mathcal{H}_i| > \frac{1}{N}\sum_{j=1}^N |\mathcal{H}_j|
\end{equation}

The gradient preservation follows from the higher sensitivity to local features in the block-wise loss.
\end{proof}

\begin{corollary}[Feature Preservation Guarantee]
Under the conditions of Theorem \ref{theorem-block-loss}, for any bathymetric feature with characteristic scale $s < |b_i|$, the block-wise loss preserves the feature with probability:
\begin{equation}
    P(\text{preserved}|s,b_i) \geq 1 - \exp(-U_i \cdot s/|b_i|)
\end{equation}
whereas the global loss preservation probability is bounded by:
\begin{equation}
    P(\text{preserved}|s) \leq 1 - \exp(-U_g \cdot s/|\mathcal{X}|)
\end{equation}
\end{corollary}

\begin{lemma}[Adaptive Capacity Allocation]
For a model with total capacity $C$ and $N$ blocks, let:
\begin{itemize}
    \item $c_i$ be the capacity allocated to block $i$
    \item $\epsilon_i(c)$ be the reconstruction error with capacity $c$
    \item $U_i$ be the block uncertainty
\end{itemize}
The block-wise uncertainty leads to optimal capacity allocation:
\begin{equation}
    c_i^* = C \cdot \frac{U_i}{\sum_j U_j}
\end{equation}
minimizing the total weighted error:
\begin{equation}
    \sum_{i=1}^N U_i \cdot \epsilon_i(c_i)
\end{equation}
\end{lemma}

\begin{proof}
The optimal allocation follows from the Karush-Kuhn-Tucker conditions with the constraint:
\begin{equation}
    \sum_{i=1}^N c_i = C
\end{equation}
and the monotonicity of $\epsilon_i(c)$ with respect to capacity.
\end{proof}

\subsection{Block-wise Uncertainty Awareness Training Mechanism}

\begin{lemma}[Convergence of Block-wise Error Tracking]
\label{block-wise-convergence}

For a given block $b_i$ in the spatial decomposition of the bathymetric prediction space, let:
\begin{itemize}
    \item $e_{t,i}$ be the instantaneous reconstruction error for block $i$ at time step $t$
    \item $\text{EMA}^{(t)}_i$ be the exponential moving average at time $t$
    \item $\mu_i$ be the true expected reconstruction error for block $i$
    \item $\sigma^2_i$ be the variance of instantaneous errors in block $i$
    \item $\alpha \in (0,1)$ be the EMA decay factor
\end{itemize}

The exponential moving average (EMA) of reconstruction errors converges to a stable estimate under the following conditions:
\begin{enumerate}
    \item The learning rate is sufficiently small
    \item The EMA decay factor $\alpha \in (0,1)$
    \item The model parameters are updated through stochastic gradient descent
\end{enumerate}
\end{lemma}

\begin{proof}
First, we define the instantaneous reconstruction error $e_{t,i}$ for block $i$ at time $t$ as:
\begin{equation}
    e_{t,i} = \frac{1}{|b_i|}\sum_{x,y\in b_i}|f(x,y) - \hat{f}(x,y)|
\end{equation}
where:
\begin{itemize}
    \item $f(x,y)$ is the true bathymetry value at position $(x,y)$
    \item $\hat{f}(x,y)$ is the predicted bathymetry value at position $(x,y)$
    \item $|b_i|$ is the number of points in block $i$
\end{itemize}

Using this, the EMA update equation can be written more compactly as:
\begin{equation}
    \text{EMA}^{(t)}_i = \alpha\text{EMA}^{(t-1)}_i + (1-\alpha)e_{t,i}
\end{equation}

We can express the expected value of the EMA:
\begin{equation}
    \mathbb{E}[\text{EMA}^{(t)}_i] = \alpha^t\text{EMA}^{(0)}_i + (1-\alpha)\sum_{k=0}^{t-1}\alpha^k \mu_i
\end{equation}

As $t \to \infty$, this converges to the true expected error:
\begin{equation}
    \lim_{t\to\infty}\mathbb{E}[\text{EMA}^{(t)}_i] = \mu_i
\end{equation}

The variance of the estimate is bounded by:
\begin{equation}
    \text{Var}[\text{EMA}^{(t)}_i] \leq \frac{(1-\alpha)^2\sigma^2_i}{1-\alpha^2}
\end{equation}
where $\sigma^2_i$ represents the variance of instantaneous errors in block $i$.
\end{proof}

\begin{lemma}[Calibrated Uncertainty Estimates]
\label{lemma-calibrated-uncertainty-estimates} 
Let:

\begin{itemize}
    \item $\alpha \in (0,1)$ be a desired confidence level
    \item $\text{EMA}_{i,1-\alpha}$ be the $(1-\alpha)$-quantile of the historical error distribution
    \item $\epsilon > 0$ be a small constant for numerical stability
    \item $\mathcal{C}_i(\alpha)$ be the empirical coverage probability
\end{itemize}
The block-wise uncertainty scores derived from the EMA tracking mechanism provide calibrated prediction intervals under the following conditions:
\begin{enumerate}
    \item The model is trained to convergence
    \item The block size is appropriately chosen relative to the spatial correlation length of bathymetric features
    \item The confidence level $\alpha$ is properly set
\end{enumerate}
\end{lemma}

\begin{proof}
For a given block $i$, we compute the uncertainty score as:
\begin{equation}
    U_i = \frac{\text{block\_error}_i}{\text{EMA}_{i,1-\alpha} + \epsilon}
\end{equation}

The empirical coverage probability $\mathcal{C}_i(\alpha)$ represents the proportion of true bathymetry values falling within the predicted confidence intervals at level $\alpha$. We can prove:
\begin{equation}
    \lim_{n\to\infty} \mathbb{P}(|\mathcal{C}_i(\alpha) - \alpha| > \epsilon) = 0
\end{equation}
where $n$ is the number of training samples.
\end{proof}

\begin{theorem}[Optimality of Block-wise Training]
\label{theorem-1}

Let:
\begin{itemize}
    \item $\theta$ be the model parameters
    \item $D(z_q)$ be the decoder output for quantized latent code $z_q$
    \item $\lambda_s, \lambda_c, \lambda_d$ be positive weighting coefficients
    \item $\mathcal{L}_{vq}$ be the vector quantization loss
    \item $\mathcal{L}_{div}$ be the codebook diversity loss
\end{itemize}
The block-wise uncertainty-aware training mechanism leads to an optimal allocation of model capacity across spatial regions under the following conditions:
\begin{enumerate}
    \item The loss function incorporates uncertainty-weighted reconstruction error
    \item The model has sufficient capacity
    \item The training process reaches convergence
\end{enumerate}
\end{theorem}

\begin{proof}
The complete training objective is:
\begin{equation}
    \mathcal{L} = \sum_i U_i \cdot |D(z_q)_i - x_i|^2 + \lambda_s(1 - \text{SSIM}(D(z_q), x)) + \lambda_c\mathcal{L}_{vq} + \lambda_d\mathcal{L}_{div}
\end{equation}

At optimality, the gradient with respect to model parameters vanishes:
\begin{equation}
    \frac{\partial\mathcal{L}}{\partial\theta} = 0
\end{equation}

This leads to the balance equation for each block:
\begin{equation}
    \frac{\partial}{\partial \theta}|D(z_q)_i - x_i|^2 = -\frac{U_i}{\lambda_s}\frac{\partial}{\partial \theta}\text{SSIM}(D(z_q), x)
\end{equation}
\end{proof}

\begin{corollary}[Error Bounds]
Under the conditions of Theorem \ref{theorem-1}, let $C$ be a constant depending on model capacity and training setup. Then for any block $i$, the expected reconstruction error is bounded by:
\begin{equation}
    \mathbb{E}[|D(z_q)_i - x_i|^2] \leq \frac{C}{U_i}
\end{equation}
\end{corollary}

\subsection{Fixed Block Size Analysis}

\begin{lemma}[Block Size Trade-off]

For a fixed block size $k$ in bathymetric enhancement, define:
\begin{itemize}
    \item $E_{stat}(k)$: statistical estimation error
    \item $E_{feat}(k)$: feature preservation error
    \item $E_{total}(k)$: total error
    \item $\sigma^2$: variance in depth measurements
    \item $\lambda$: constant related to bathymetric feature density
\end{itemize}
There exists a fundamental trade-off:
\begin{equation}
    E_{total}(k) = \underbrace{\frac{\sigma^2}{k^2}}_{E_{stat}(k)} + \underbrace{\lambda k}_{E_{feat}(k)}
\end{equation}
\end{lemma}

\begin{proof}
The statistical error follows from the variance of the sample mean:
\begin{equation}
    \text{Var}[\hat{\mu}_k] = \frac{\sigma^2}{k^2}
\end{equation}

The feature preservation error grows linearly with block size due to local stationarity:
\begin{equation}
    E_{feat}(k) = \lambda k
\end{equation}

This creates a natural tension between reducing statistical error (favoring larger blocks) and preserving local features (favoring smaller blocks).
\end{proof}

\begin{theorem}[Fixed Block Size Optimality]
For a bathymetric region with:
\begin{itemize}
    \item Measurement noise variance $\sigma^2$ in the sampling process
    \item Observed bathymetric gradient characteristic $\lambda = \frac{\Delta z}{\Delta x}$
    \item Sampling resolution defined by $\Delta x$
    \item Measured depth variations $\Delta z$
\end{itemize}

The mean squared error (MSE) between estimated and true uncertainties has two components:
\begin{equation}
    \text{MSE}(k) = \mathbb{E}[(U_k - U^*)^2]
\end{equation}

Which decomposes into:
\begin{align}
    \text{MSE}(k) &= \underbrace{\frac{\sigma^2}{k^2}}_{\text{measurement noise}} + \underbrace{\left(\frac{\Delta z}{\Delta x} k\right)^2}_{\text{structural variation}} \\
    &= \frac{\sigma^2}{k^2} + (\lambda k)^2
\end{align}

The block size $k^*$ that minimizes this error is:
\begin{equation}
    k^* = \left(\frac{\sigma^2}{2(\Delta z/\Delta x)^2}\right)^{1/4}
\end{equation}

This optimal block size reflects the balance between:
\begin{itemize}
    \item Reducing measurement noise effects ($\sim 1/k^2$ term)
    \item Preserving observed bathymetric structures ($\sim k^2$ term)
\end{itemize}
\end{theorem}

\begin{proof}
The measurement noise component follows from sampling theory and the Central Limit Theorem:
\begin{equation}
    \text{Var}[U_k] = \frac{\sigma^2}{k^2}
\end{equation}

The structural variation term arises from the observed bathymetric gradients in the data:
\begin{equation}
    \text{Bias}^2[U_k] = \left(\frac{\Delta z}{\Delta x} k\right)^2
\end{equation}

The optimal block size is found by minimizing total MSE:
\begin{equation}
    \frac{d}{dk}\text{MSE}(k) = -\frac{2\sigma^2}{k^3} + 2\left(\frac{\Delta z}{\Delta x}\right)^2k = 0
\end{equation}

Solving yields the optimal $k^*$.
\end{proof}

\begin{remark}
The optimal fixed block size $k^*$ represents a global compromise between measurement noise reduction and bathymetric structure preservation. While individual regions may have different local characteristics (some being steeper, others flatter), this $k^*$ provides the best fixed-size choice that minimizes the overall expected error across the entire domain.
\end{remark}


\begin{corollary}[Error Bound]
For any fixed block size $k$, the uncertainty estimation error satisfies:
\begin{equation}
    \text{MSE}(k) \leq \min\left(\frac{\sigma^2}{k^2}, (\lambda k)^2\right)
\end{equation}
with equality when the feature scale matches the block size.
\end{corollary}

\begin{lemma}[Convergence Rate]
Let:
\begin{itemize}
    \item $\alpha$ be the EMA decay factor
    \item $\text{EMA}^*$ be the true uncertainty
\end{itemize}
With fixed block size $k$, the EMA-based uncertainty tracking converges at rate:
\begin{equation}
    \|\text{EMA}^{(t)} - \text{EMA}^*\|_2 \leq (1-\alpha)^t\|\text{EMA}^{(0)} - \text{EMA}^*\|_2
\end{equation}
\end{lemma}

\begin{proof}
From the EMA update equation:
\begin{equation}
    \text{EMA}^{(t)} = \alpha\text{EMA}^{(t-1)} + (1-\alpha)\text{error}^{(t)}
\end{equation}

The convergence follows from the contraction mapping principle since $\alpha \in (0,1)$.
\end{proof}

\begin{theorem}[Consistency]
Let $T$ be the number of training iterations. The fixed block size uncertainty estimator is consistent if for any $\epsilon > 0$:
\begin{equation}
    \lim_{T\to\infty}\mathbb{P}(|\hat{U}_k - U^*| > \epsilon) = 0
\end{equation}
\end{theorem}

\subsection{VQ-VAE Specific Analysis}

\begin{lemma}[Enhanced Uncertainty Quantification in VQ-VAE]

Let:
\begin{itemize}
    \item $C = \{e_k\}_{k=1}^K$ be the codebook with $K$ entries
    \item $z$ be the encoder output
    \item $z_q$ be the quantized latent code
    \item $W$ be the CNN weight matrix
    \item $D$ be the discriminator
\end{itemize}
The block-wise uncertainty mechanism achieves superior performance in VQ-VAE compared to continuous latent space models (CNN, ESRGAN) due to:
\begin{enumerate}
    \item Discrete Codebook Quantization
    \item Local Feature Preservation
    \item Bounded Representation Error
\end{enumerate}
\end{lemma}

\begin{proof}
The quantization operation maps continuous encoder outputs to discrete codebook entries:
\begin{equation}
    z_q = e_k, \text{ where } k = \argmin_i \|z - e_i\|_2
\end{equation}

For any block $b_i$, we have:
\begin{equation}
    \mathbb{P}(\text{error}_i > \epsilon) \leq \sum_{k=1}^K \mathbb{P}(\text{error}_i > \epsilon | z_q = e_k)\mathbb{P}(z_q = e_k)
\end{equation}

The VQ-VAE architecture preserves local features:
\begin{equation}
    \text{Features}(b_i) = \text{Decoder}(z_q + \text{ResidualAttention}(z))
\end{equation}

The block-wise uncertainty decomposes as:
\begin{equation}
    U_i = f(\text{local\_structure}_i, \text{codebook\_assignment}_i)
\end{equation}

This improves upon continuous models:
\begin{align}
    U_i^{\text{CNN}} &= f(\text{conv\_features}_i) \\
    U_i^{\text{GAN}} &= f(\text{adversarial\_features}_i)
\end{align}

The representation error is bounded:
\begin{equation}
    \|\hat{x} - x\|_2^2 \leq \min_{k} \|e_k - z\|_2^2 + \|\text{Decoder}(e_k) - x\|_2^2
\end{equation}

Leading to tighter uncertainty bounds:
\begin{equation}
    \text{Var}[U_i^{\text{VQ-VAE}}] \leq \frac{(1-\alpha)^2\sigma_i^2}{1-\alpha^2} \cdot \min_{k} \|e_k - z\|_2^2
\end{equation}

Compared to traditional approaches:
\begin{align}
    \text{Var}[U_i^{\text{CNN}}] &\leq \frac{(1-\alpha)^2\sigma_i^2}{1-\alpha^2} \cdot \|W\|_2^2 \\
    \text{Var}[U_i^{\text{GAN}}] &\leq \frac{(1-\alpha)^2\sigma_i^2}{1-\alpha^2} \cdot (1 + \|\nabla_D\|_2^2)
\end{align}
\end{proof}

\begin{theorem}[Optimality of VQ-VAE Uncertainty]

Let:
\begin{itemize}
    \item $U_i^*$ be the true uncertainty for block $i$
    \item $U_i^{\text{other}}$ be uncertainty estimates from other models
    \item $\bar{U}_i$ be the mean uncertainty for block $i$
\end{itemize}
The block-wise uncertainty mechanism in VQ-VAE achieves optimal uncertainty estimation:
\begin{equation}
    \mathbb{E}[\|U_i^{\text{VQ-VAE}} - U_i^*\|_2^2] \leq \mathbb{E}[\|U_i^{\text{other}} - U_i^*\|_2^2]
\end{equation}
\end{theorem}

\begin{proof}
For any block $b_i$, we can decompose the expectation:
\begin{align}
    \mathbb{E}[\|U_i^{\text{VQ-VAE}} - U_i^*\|_2^2] &= \sum_{k=1}^K \mathbb{P}(z_q = e_k)\mathbb{E}[\|U_i^{\text{VQ-VAE}} - U_i^*\|_2^2 | z_q = e_k] \\
    &\leq \min_{k} \|e_k - z\|_2^2 \cdot \mathbb{E}[\|U_i^* - \bar{U}_i\|_2^2]
\end{align}
where the inequality follows from the optimality of codebook quantization.
\end{proof}

\begin{corollary}[Calibration Guarantee]
For a desired confidence level $\alpha$, the VQ-VAE uncertainty mechanism provides better-calibrated uncertainty estimates:
\begin{equation}
    |\mathbb{P}(|x - \hat{x}| \leq U_i^{\text{VQ-VAE}}) - \alpha| \leq |\mathbb{P}(|x - \hat{x}| \leq U_i^{\text{other}}) - \alpha|
\end{equation}
This indicates that VQ-VAE uncertainty estimates achieve coverage probabilities closer to the nominal confidence level.
\end{corollary}

